SkipCat: Rank-Maximized Low-Rank Compression of Large Language Models via Shared Projection and Block Skipping

Large language models (LLM) have achieved remarkable performance across a wide range of tasks. However, their substantial parameter sizes pose significant challenges for deployment on edge devices with limited computational and memory resources. Low-rank compression is a promising approach to address this issue, as it reduces both computational and memory costs, making LLM more suitable for resource-constrained environments. Nonetheless, na\"ive low-rank compression methods require a significant reduction in the retained rank to achieve meaningful memory and computation savings. For a low-rank model, the ranks need to be reduced by more than half to yield efficiency gains. Such aggressive truncation, however, typically results in substantial performance degradation. To address this trade-off, we propose SkipCat, a novel low-rank compression framework that enables the use of higher ranks while achieving the same compression rates. First, we introduce an intra-layer shared low-rank projection method, where multiple matrices that share the same input use a common projection. This reduces redundancy and improves compression efficiency. Second, we propose a block skipping technique that omits computations and memory transfers for selected sub-blocks within the low-rank decomposition. These two techniques jointly enable our compressed model to retain more effective ranks under the same compression budget. Experimental results show that, without any additional fine-tuning, our method outperforms previous low-rank compression approaches by 7% accuracy improvement on zero-shot tasks under the same compression rate. These results highlight the effectiveness of our rank-maximized compression strategy in preserving model performance under tight resource constraints.

==> table/bigO.tex <==

\begin{table}[!htbp]
    \centering
    \begin{tabular}{c|c}
    \toprule
        & Time and Space Complexity \\
    \midrule
        Baseline  & $\mathcal{O} (Cd_{\mathrm{in}}d_{\mathrm{out}})$ \\
        Naïve  & $\mathcal{O} (Cr(d_{\mathrm{in}}+d_{\mathrm{out}}))$ \\
        Cat & $\mathcal{O} (r(d_{\mathrm{in}}+Cd_{\mathrm{out}}))$ \\
        Skip  & $\mathcal{O} (Cr(d_{\mathrm{in}}+d_{\mathrm{out}}-r))$ \\
        SkipCat  & $\mathcal{O} (r(d_{\mathrm{in}}+Cd_{\mathrm{out}}-r))$ \\
    \bottomrule
    \end{tabular}
    \caption{Time and memory complexity of standard weight multiplication (Baseline), its naïve low-rank approximation (Naïve), matrix concatenation (Cat), block skipping (Skip), and our proposed SkipCat. Here, $r$ denotes the rank, $d_{\mathrm{in}}$ and $d_{\mathrm{out}}$ are the input and output dimensions, respectively, and $C$ is the number of concatenated matrices. SkipCat reduces both floating‐point operations (FLOPs) and memory requirements compared to the other methods.}

    \label{tab:flops}
\end{table}



% \begin{table}[!htbp]
%     \centering
%     \begin{tabular}{c|cc}
%     \toprule
%         & FLOPs & \#Params \\
%     \midrule
%         Baseline  & $2d_{\mathrm{in}}d_{\mathrm{out}}$ & $d_{\mathrm{in}}d_{\mathrm{out}}$ \\
%         Naïve  & $2r(d_{\mathrm{in}}+d_{\mathrm{out}})$ & $r(d_{\mathrm{in}}+d_{\mathrm{out}})$ \\
%         Skip  & $2r(d_{\mathrm{in}}+2d_{\mathrm{out}}-r)+r$ & $r(d_{\mathrm{in}}+d_{\mathrm{out}}-r)$ \\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison of computational costs for standard weight multiplication (Baseline), its low-rank approximation (LR), and the proposed Schur method. The Schur method achieves fewer floating‐point operations (FLOPs) and a reduced parameter count compared to baseline and LR.}
%     \label{tab:flops2}
% \end{table}



